PURL: Safe and Effective Sanitization of Link Decoration

While privacy-focused browsers have taken steps to block third-party cookies and mitigate browser fingerprinting, novel tracking techniques that can bypass existing countermeasures continue to emerge. Since trackers need to share information from the client-side to the server-side through link decoration regardless of the tracking technique they employ, a promising orthogonal approach is to detect and sanitize tracking information in decorated links. To this end, we present PURL (pronounced purel-l), a machine-learning approach that leverages a cross-layer graph representation of webpage execution to safely and effectively sanitize link decoration. Our evaluation shows that PURL significantly outperforms existing countermeasures in terms of accuracy and reducing website breakage while being robust to common evasion techniques. PURL's deployment on a sample of top-million websites shows that link decoration is abused for tracking on nearly three-quarters of the websites, often to share cookies, email addresses, and fingerprinting information.

==> extras/comments.tex <==
% Dash command
\newcommand*\dash{\unskip\kern.16667em---\penalty\exhyphenpenalty
        \hskip.16667em\relax
}

 \marginparwidth.25in
 % Complex \xxx for making notes of things to do. 
  % Puts text in brackets and in bold font, and normally adds a marginpar
 % with the text ``xxx'' so that it is easy to find.  On the other hand, if
 % the comment is in a minipage, figure, or caption, the xxx goes in the text,
 % because marginpars are not possible in these situations.
 {\makeatletter
  \gdef\xxxmark{%
    \expandafter\ifx\csname @mpargs\endcsname\relax % in minipage?
      \expandafter\ifx\csname @captype\endcsname\relax % in figure/caption?
        \marginpar{\textcolor{red}{xxx}}% not in a caption or minipage, can use marginpar
      \else
        \textcolor{red}{xxx~}% notice trailing space
      \fi
    \else
      \textcolor{red}{xxx~}% notice trailing space
    \fi}
  \gdef\xxx{\@ifnextchar[\xxx@lab\xxx@nolab}
  \long\gdef\xxx@lab[#1]#2{{\bfseries [\xxxmark \textcolor{red}{#2}
  ---{\scshape #1}]}}
  \long\gdef\xxx@nolab#1{{\bfseries [\xxxmark \textcolor{red}{#1}]}}
  % This turns them off:
     % \long\gdef\xxx@lab[#1]#2{}\long\gdef\xxx@nolab#1{}
 }
 
 \marginparwidth.25in
 % Complex \yyy for making notes of things to do.
 % Puts text in brackets and in bold font, and normally adds a marginpar
 % with the text ``yyy'' so that it is easy to find.  On the other hand, if
 % the comment is in a minipage, figure, or caption, the yyy goes in the text,
 % because marginpars are not possible in these situations.
 {\makeatletter
  \gdef\yyymark{%
    \expandafter\ifx\csname @mpargs\endcsname\relax % in minipage?
      \expandafter\ifx\csname @captype\endcsname\relax % in figure/caption?
        \marginpar{\textcolor{blue}{yyy}}% not in a caption or minipage, can use marginpar
      \else
        \textcolor{blue}{yyy~}% notice trailing space
      \fi
    \else
      \textcolor{blue}{yyy~}% notice trailing space
    \fi}
  \gdef\yyy{\@ifnextchar[\yyy@lab\yyy@nolab}
  \long\gdef\yyy@lab[#1]#2{{\bfseries [\yyymark \textcolor{blue}{#2}
  ---{\scshape #1}]}}
  \long\gdef\yyy@nolab#1{{\bfseries [\yyymark \textcolor{blue}{#1}]}}
  % This turns them off:
%   \long\gdef\yyy@lab[#1]#2{}\long\gdef\yyy@nolab#1{}%
 }
 
  \marginparwidth.25in
 % Complex \zzz for making notes of things to do.
 % Puts text in brackets and in bold font, and normally adds a marginpar
 % with the text ``zzz'' so that it is easy to find.  On the other hand, if
 % the comment is in a minipage, figure, or caption, the zzz goes in the text,
 % because marginpars are not possible in these situations.
 {\makeatletter
  \gdef\zzzmark{%
    \expandafter\ifx\csname @mpargs\endcsname\relax % in minipage?
      \expandafter\ifx\csname @captype\endcsname\relax % in figure/caption?
        \marginpar{\textcolor{green}{zzz}}% not in a caption or minipage, can use marginpar
      \else
        \textcolor{green}{zzz~}% notice trailing space
      \fi
    \else
      \textcolor{green}{zzz~}% notice trailing space
    \fi}
  \gdef\zzz{\@ifnextchar[\zzz@lab\yyy@nolab}
  \long\gdef\zzz@lab[#1]#2{{\bfseries [\zzzmark \textcolor{green}{#2}
  ---{\scshape #1}]}}
  \long\gdef\zzz@nolab#1{{\bfseries [\zzzmark \textcolor{green}{#1}]}}
  % This turns them off:
  % \long\gdef\zzz@lab[#1]#2{}\long\gdef\zzz@nolab#1{}%
 }

\iffalse %\iftrue to turn on

% Squeeze space on paragraphs
\renewcommand{\paragraph}[1]{\vspace{0.1in}\noindent\textbf{#1.}}
\newcommand{\iparagraph}[1]{\vspace{0.08in}\noindent\textit{#1.}}
%\newcommand{\qiparagraph}[1]{\vspace{0.1in}\noindent\textit{#1}}

%%%%% Squeeze space on enumerations
\makeatletter
\def\@listi{\leftmargin\leftmargini
    \parsep 1\p@ \@plus0\p@ \@minus\p@
    \topsep 2\p@   \@plus0\p@ \@minus\p@
%    \topsep 2\p@   \@plus2\p@ \@minus2\p@
%    \itemsep1.25\p@ \@plus\p@ \@minus\p@}
    \itemsep1\p@ \@plus0\p@ \@minus\p@}
\let\@listI\@listi\@listi
\makeatother

\newcommand{\edits}[1]{\textcolor{blue}{#1}}

\fi


==> graveyard/background.tex <==
% \subsection{Adoption of Link Decoration for Tracking}
% The concept of link decoration in URLs was first introduced in the early days of the World Wide Web in the 90s. In his book \textit{Weaving the Web}, Tim Berners-Lee reveals that the first version of the HTTP protocol, HTTP/0.9 introduced in 1991, did not support query parameters \cite{berners1999weaving}. However, they were later added as part of the HTTP/1.0 protocol, by Berners-Lee et al., released in 1996 \cite{rfc1945}, for enabling more complex interactions between clients and servers \cite{berners1999weaving, rfc1866}. As the web grew more complex, URL query parameter syntax was later refined, as part of RFC 3986 section 3.4 released January 2005, by Berners-Lee et al. as the URI segment appearing after the `?' and carrying identifying information in the form of `key=value' utilizing delimiters like `\&', `;', or `,'.

% However, the usage of URL decoration quickly diverged from just ``passing additional data'' in HTTP requests. In 1996, \textit{e.g. Software Inc.} released \textit{WebTrends} which is widely regarded as the first web analytics software \cite{webtrends1996}. \textit{Webtrends} used the \textit{WT.mc\_id} query parameter to track clicks and site visits, across multiple marketing campaigns\cite{webtrends1996}.

% In recent years, thanks to the omnipresent online tracking and advertising services, web users are constantly targeted for their personal information - often without their explicit consent. URL decoration, as a means of tracking, has become a favorable choice for trackers due to its ease of use compared to cookies or fingerprinting, which require additional handling and setup on the client and server sides. One such case is the UID \textit{smuggling} \cite{randall2022measuring}, which is an emerging tracking technique geared towards evading current privacy protections. UID \textit{smuggling} works by inserting user identifiers (UIDs) in a user's web navigation request. This allows trackers to synchronize UIDs and, hence, gain the ability to track users across sites. Although this paper, by Randal et al., conjectures that UIDs for individual users remain the same across sites, as will be shown in this work, for instance, the \texttt{fbp} identifier is chosen randomly from 50 identifiers and changes for the same user again and again.

\subsection{Countermeasures against Link Decoration}
There have been different efforts across academia and the industry to mitigate attempts of tracking through link decoration. We look at these approaches in the following subsections.
\subsubsection{Deployed Countermeasures}
THe app
These include privacy-enhancing features in browsers such as Brave and Mozilla Firefox~\cite{brave2020grab, brave2023hacks, firefoxquerystripping}, and extensions such as uBlock Origin~\cite{gorhilluBlockCommit}. We describe these in more detail below:


\para{Safari}. Rather than actively filtering tracking parameters from URL queries, Safari, starting with \textit{Intelligent Tracking Prevention (ITP) 2.2}, caps persistent cookies set through \texttt{document.cookie} to 1 day of storage when both of the following conditions are met:
\begin{itemize}
    \item A domain classified with cross-site tracking capabilities was responsible for navigating the user to the current webpage
    \item The final URL of the navigation mentioned above has a query string and/or a fragment identifier
\end{itemize} 
as stated in ITP 2.2 specs \cite{itp2.2}. However, many trackers switched to using other browser storage mechanisms, such as \textit{localStorage}, as no restrictions on expiry time were set there. Also, trackers opted to decorating an intermediate page instead of decorating the destination URL. The decorated link would be accessed via \texttt{document.referrer} on the destination page. Hence, Safari, starting with \textit{ITP 2.3}, mitigates such efforts as follows \cite{wilander2.3}:
\begin{itemize}
    \item \texttt{website.example} is marked for non-cookie website data deletion if the user is navigated from a domain classified with cross-site tracking capabilities to a final URL with a query string and/or a fragment identifier, such as \newline \texttt{website.example?clickID=0123456789}
    \item After 7 days of Safari use without the user interacting with a webpage on \texttt{website.example}, all of \texttt{website.example}’s non-cookie website data is deleted
\end{itemize}
Hence, \textit{ITP 2.3} effectively caps lifetime for all script-writable data if the user is navigated with link decoration from a classified domain. However, it is important to note that \textit{ITP} does not actively sanitize URLs. Its efforts are concentrated on capping expiry times and limiting access to various pieces of website data.

\para{Brave}. Since 20 July 2020\cite{brave2020grab}, Brave removes known tracking parameters from URLs by matching them against a list of known tracking parameters. These parameters are determined from the documentation provided by the trackers themselves, through crowd-sourced tracker lists, and from encounters by Brave developers and users. Brave's list of removed query parameters can be found in their source code \cite{brave2023hacks,brave2023filter}. The list includes popular tracking parameters like \texttt{fbclid}, \texttt{gclid}, \texttt{msclkid}, \texttt{mceid}, and...

\para{Firefox}. First introduced in Firefox Nightly 96 \cite{mozillanightly}, Mozilla integrated the \textit{Query Parameter Stripping} feature as part of Firefox 102.0 released June 28, 2022 \cite{mozilla2022firefox}. However, users would have to enable \textit{Enhanced Tracking Prevention} in the \textit{Privacy \& Security} tab besides setting the security level to \textit{Strict} for the URL sanitization to work. Firefox also uses a static \texttt{stripList} to filter parameters like \texttt{gclid}, \texttt{dclicd}, \texttt{msclkid}, \texttt{\_openstat}, \texttt{yclid}, \texttt{wickedid}, and... \cite{firefoxquerystripping}

\para{uBlock Origin}. Although uBlock Origin (uBO) developers were originally hesitant to actively sanitize URL query strings due to feature creep and performance issues \cite{uBOHesitant1, uBOHesitant2}, uBO eventually introduced the \texttt{removeparam} feature in its 1.32.0 version release \cite{gorhilluBlockCommit}. The URL-parameter-stripping feature works by intercepting web requests, parsing the intercepted URL, and identifying tracking parameters. If uBO detects any tracking parameters in the URL, it removes them and any associated values. For example, if the URL contains the tracking parameter \texttt{"?utm\_source=google"}, uBO will remove this parameter and leave only the base URL. Once uBO has stripped any tracking parameters from the URL, it modifies the request to remove the tracking parameters before sending it to the server hosting the website. uBO uses a manually-crafted list of query parameters, utilizing string- and regular expression-matching, to identify and sanitize URL query parameters \cite{gorhilluBlockCommit}.


As was observed, many browsers and extensions rely on filter-based content blocking for their URL query parameter sanitization measures. The problem with such an approach is that such lists are mostly manually-crafted, static, and require frequent maintenance. Hence, such rules could be too restrictive, i.e., content blocking rules break benign websites; or too relaxed, i.e., user privacy is violated due to unobserved tracking content. This makes filter list authors very reluctant to add additional parameters to their filters due to fear of breakage. Moreover, manually-crafted filter lists do not seem scalable at all. 

\subsubsection{Countermeasures proposed by prior research}
%

As of this writing, path parameter based tracking and sanitization has not been researched extensively as this paper is the first such work to study and mitigate path parameter tracking. However, existing work has considered smuggling of identifiers through query parameters.
\xxx[Umar]{The last sentence needs elaboration. Also, is it the only paper which discusses link decoration? or the exfiltration of identifiers in the URLs? }


% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=\linewidth, trim={0.7cm 3cm 0.7cm 4.5cm},clip]{figures/link-dedecor-timeline.png}
%     \caption{URL Parameters Timeline}
%     \label{fig:url_parameters_timeline}
% \end{figure*}



\Ht{Show example of resource path based tracking link decorations: (either background or the ground truth labeling)
example.com/XXXXXX/content/script.js

example.com/YYYYYY/content/script.js
}

==> graveyard/background_related_work.tex <==
In this section, we discuss preliminaries, review related work, and survey existing countermeasures against the abuse of link decoration for tracking in industry and academia. 
% \xxx[Umar]{It occurred to me here that the link decoration is not clearly defined in introduction. I know we present a formal definition in this section but a one line summary/definition in introduction would provide readers some context.}
% \xxx[Shaoor]{I think the current description as "decorated" links would suffice for the introduction with more in-depth detail in this section}{}

\subsection{What is Link Decoration?}
A URL is composed of the following key components:, scheme, fully qualified domain name (FQDN), resource path, query parameters, and fragments.
%
We use \texttt{\textcolor{blue}{https}://\textcolor{green}{a.site.example}/\textcolor{violet}{YYY/ZZZ/}\textcolor{magenta}{pixel.jpg}?\\\textcolor{red}{ISBN=XXX\&UID=ABC123}\#\textcolor{orange}{xyz}}, as an example URL to define these segments below:

%%
\para{Base URL}. \texttt{\textcolor{blue}{https://}} is the scheme in this URL and \texttt{\textcolor{green}{a.site.example}} is the FQDN. These segments are combined to form the base URL.  


\para{Resource path}. Immediately following the FQDN, \texttt{\textcolor{violet}{/YYY/ZZZ}} is the resource path in the URL. 
%
It points to a directory, file, API endpoint, or other resource on the server. 
%
\texttt{\textcolor{magenta}{pixel.jpg}} is the name of the resource hosted on the server. 


%%
\para{Query parameters}. Immediately following the resource path after the \textit{?} delimiter, \texttt{\textcolor{red}{ISBN=XXX\&UID=abc123}} are the query parameters in the URL. 
%
A query parameter consists of a key-value pair, where the key is separated from the value by the \textit{=} delimiter.
%
Multiple query parameters in a URL are separated from each other by the \textit{\&} delimiter.


%%
\para{Fragments}. Immediately following the query parameters after the \textit{\#} delimiter, \texttt{\textcolor{orange}{xyz}} is the fragment in the URL. 
%
Fragments can be a singular value or multiple key-value pairs that are separated by the \& delimiter (similar to query parameters).\footnote{In cases where fragments contain multiple key-value pairs, we treat these key-value pairs similarly as query parameters to facilitate easier comparison and analysis across different parts of URL.}


%%
While only query parameters are traditionally considered as link decoration~\cite{}, we find that link decoration can be carried out using the resource path, query parameters, and fragments (discussed further in Section~\ref{subsec: methodology})\footnote{While fragments are not sent alongside a request to a server, the server can send a redirect to another page, which can access the fragments from the URL, e.g., through JavaScript APIs.}. Next, we describe the threat model we consider for tracking through link decoration.
\subsection{Threat Model}
\label{app:threat_model}

Our threat model focuses on the exfiltration of identifiable user information through link decoration via third-party requests.
%
We exclude first-party requests from our analysis as first parties use this information to provide key website functionality.
%
Our threat model does not differentiate between same-site, same-site-cross-domain, or cross-site tracking, as previous research \cite{Munir23CookieGraphArxiv} has shown that exfiltration of information such as cookies and fingerprints can be used for either category of tracking depending on type of information collected (third-party cookie vs first-party cookie, fingerprints, etc.), number of websites the tracker collects this information on, and extent of information sharing between different trackers.
%
We consider two main entities in our threat model: the victim (users), and the adversary (trackers).
%
While exfiltration of some information such as first-party cookies requires deliberate collusion between trackers and the website publisher \cite{Sanchez2021JourneyToCookies, Munir23CookieGraphArxiv}, we do not consider the publisher to be an active part of the threat model.
%%

\textbf{We assume that the victim:}
%
\begin{itemize}
    \item visits different websites using one or more devices (desktop/mobile)
    \item has third-party and first-party enabled
    \item provides personally identifiable information (PII) such as email address on these websites
\end{itemize}
%
\textbf{We assume that the adversary:}
%
\begin{itemize}
    \item is present in either a third-party (can set and read third-party cookies) or a first-party (can set and read first-party cookies) context on the websites that the victim visits
    \item can collect and exfiltrate information such as third-party/first-party cookies, email address, \etc, which can be used for user identification
\end{itemize}

The adversary uses link decorations to exfiltrate user information to track user activity, as described below:
%%

A user visits a website \textit{example.com}, where tracker A is present in a third-party context, while tracker B is present in a first-party context.
%
The user provides their email on the website, while both tracker A and tracker B set their corresponding third- and first-party cookies.
%
Tracker A sends the email to its own server by appending it as a link decoration in the request URL.
%
Third-party cookies set by tracker A are automatically sent alongside the request.
%
In addition to the email, tracker B also appends the first-party cookies set alongside the request URL as first-party cookies are not automatically sent to any domain other than the first-party domain.
%%

Both tracker A and B also send information to tracker C, which has a data sharing agreement with these trackers.
%
Both trackers A and B append their cookies along with the user email with the request sent to tracker C.
%
This information exfiltration by tracker A and B to their own servers, along with those hosted by tracker C, allows the user to be tracked on different sites that the user visits where these trackers are also present.

% as we discuss later in , link decoration more broadly encompasses 
%%
\subsection{Abuse of Link Decorations for Tracking}
% Link decorations can either be used to implement benign functionality or used for tracking. 
%
The abuse of link decoration for online tracking is not a new phenomenon. 
%
The first record on link decoration abuse is from 1996, when {Webtrends} (an analytics service) used the \texttt{WT.mc\_id} query parameter for click tracking in advertising campaigns \cite{webtrends1996, webtrends-documentation}.
%
Since then, link decorations in general, and query parameters specifically, have been widely used for creating personalized links to track the success of advertising campaigns.
%
For example, Urchin Tracking Module (UTM) parameters, such as \texttt{utm\_source}, are link decorations that identify the source of traffic on a website and attribute it to specific advertising campaigns.~\cite{GoogleUTM, HubspotUTM, MailchimpUTM, MonsterinsightsUTM}.
\xxx[Umar]{I thought this example was in support of the previous sentence but it does not seem to support the key point of the previous sentence.}{}
\xxx[Shaoor]{UTMs are used for tracking the success of advertising campaigns, I changed the sentence a little bit to make it more obvious.}

%%
Prior research has documented the abuse of link decorations in various tracking techniques. 
%
Papadopoulos \etal showed that trackers implement cookie syncing by decorating URLs with identifiers \cite{Papadopoulos19cookiesyncing}. 
%
Iqbal \etal \cite{Iqbal22USENIXKhaleesi} showed that cookie syncers share potential identifiers through query parameters.
%
Fouad \etal \cite{Fouad20PixelsPETS} showed that trackers share identifiers through query parameters, and argue that these requests cannot be trivially blocked (e.g., using filter lists) because they sometimes fetch functional resources. 
%
While prior work has proposed approaches to detect cookie syncing, which in turn relies on link decoration, these studies do not specifically study the abuse of link decorations for tracking.
%
To the best of our knowledge, Randall \etal \cite{randall2022measuring} is the first study that specifically studies tracking query parameters. 
%
They found that 8.1\% of the navigation URLs included identifiers as query parameters for tracking.  


%%
With recent \cite{firefox-cookie-policy, safari-default-cookie} and imminent restrictions \cite{Schuh2020ChromeCookies} on third-party cookies, trackers are moving towards alternative methods of identifying users, which include the use of first-party cookies \cite{Munir23CookieGraphArxiv,ChenACM2021CookieSwapParty, Sanchez2021JourneyToCookies}, personally identifiable information (PII) \cite{acar2020no, senol2022leaky_forms}, and device/browser fingerprinting \cite{Iqbal21FingerprintingSP, Fouad22CookieRespawningPETS, laperdrix2020browser}.
%
In contrast to third-party cookies that are automatically included as headers in outgoing HTTP requests, these alternative tracking methods rely on link decoration for user information exfiltration. 
%
As trackers shift their focus towards these alternative tracking methods, it is reasonable to assume that the abuse of link decoration for tracking will also continue to increase.


%%
\subsection{Countermeasures Against the Abuse of Link Decoration for Tracking}
\label{subsection: countermeasures related work}
Given the increased focus on alternative ways to track users due to restrictions on third-party cookies, privacy-focused browsers, and browser extensions, to some extent, have started deploying countermeasures against the abuse of link decorations. 
% \xxx[Umar]{Hmm I do not think that so far with our write up, we have clearly demonstrated if the abuse of link decoration is increasing. At least I am not convinced yet. One reason I am confused is because the message from the previous sub section is not super crisp. It is taking several diversions, which could be avoided. For example, it is unclear what to take away from the urchin example, prior studies not focusing on link decoration but their results being quoted to support that link decoration is on the rise, unclear why a paper studying link decoration for the first time is of significance, missing transition between the discussion of link decoration to alternative tracking techniques,...}
% \xxx[Shaoor]{Replaced the increased abuse of link decorations with alternative ways of tracking due to restrictions on third-party cookies. This point is proved through the research quoted in the previous section. Regarding the claim in the previous section around increasing abuse of tracking link decorations, with the quoted research on other forms to tracking becoming popular and no other way for trackers to exfiltate the information without using link decorations, I think the last sentence of the section does justify why it is reasonable to assume that abuse of link decoration will also increase.}
%
Next, we describe these already deployed countermeasures as well as those proposed in prior research and highlight their limitations.  

\subsubsection{Countermeasures deployed by privacy-focused browsers}

We first survey countermeasures deployed by privacy-focused browsers against the abuse of link decoration for tracking. 
% \xxx[Umar]{It is not obvious, why the reader should care about and read specific countermeasures deployed by browsers and extensions. I am also confused about the takeaways of this and the following subsubsection. If the goal is to convey that prior solutions are based on manually curated filter lists and contain limited parameters, it is not coming across as such. I see that the subsubsection after the next mentions this point but I think this is the right place where the reader should be conveyed this information.}
% \xxx[Shaoor]{I have moved the discussion around limitation of filter lists earlier after discussing each of the countermeasures, this should provide reader immediate information about their shortcomings}

%%
\para{Brave.} Since July 2020 \cite{brave2020grab}, Brave browser attempts to remove tracking parameters from URLs by matching them against a list of known tracking parameters.
%
This filter list is curated by analyzing the documentation provided by the trackers themselves and from the reports submitted by Brave developers and users.
%
At the time of writing, Brave's filter list of tracking query parameters contains 47 query parameters \cite{brave2023hacks,brave2023filter}. 
%
%These 47 query parameters were added to the list over the course of three years, with the earliest addition in April 2019 \cite{brave-list-first-addition} and the latest update in June 2023 \cite{brave-list-update-latest}.

%and includes popular tracking parameters such as \texttt{fbclid} (Facebook), \texttt{gclid} (Google), \texttt{msclkid} (Microsoft), and \texttt{mceid} (Adobe).

%%
\para{Firefox.} In January 2022, Firefox introduced the {query parameter stripping} feature \cite{mozillanightly} in Firefox Nightly 96. 
%
Mozilla integrated this feature in Firefox 102.0 in June 2022 \cite{mozilla2022firefox} although it was not enabled by default -- Firefox users have to set \textit{Strict} security level in {Enhanced Tracking Prevention} (ETP) to enable this feature.
%
Similar to Brave, Firefox also relies on a curated filter list of tracking query parameters. 
%
At the time of writing, Firefox's filter list of tracking query parameters contains 23 query parameters \cite{firefoxquerystripping}.

% uch as gclid, dclicd, msclkid, \_openstat, yclid, and wickedid \cite{firefoxquerystripping}.


%%
\para{Safari.} Since June 2023, Safari 17 beta \cite{safari17linkdecoration} strips known tracking query parameters in Safari's private browsing mode.
%
Similar to Brave and Firefox, Safari also relies on a curated filter list of tracking query parameters. 
%
At the time of writing, Safari's filter list of tracking query parameters contains 24 query parameters \cite{privacytests}.
%%

All three browsers rely on limited, manually curated filter lists of query parameters.
%
It is well-known from prior research that filter lists are manually curated, error-prone, and slow to update \cite{Iqbal17AntiABIMC,hieu2021cv,alrizah2019errors}.

%%
\subsubsection{Countermeasures deployed by privacy-focused browser extensions}
Next, we survey countermeasures deployed by privacy-focused browser extensions against the abuse of link decoration for tracking. 


%%
\para{AdGuard.}
AdGuard introduced a new filter type named \texttt{removeparam} to remove tracking query parameters from request URLs in April 2021 \cite{adguard-url-tracking-filter}.
%
At the time of writing, AdGuard's filter list includes more than one thousand query parameter rules \cite{adguard-url-tracking-filter-general,adguard-url-tracking-filter-specific,adguard-url-tracking-filter-allowlist}. 


%%
\para{uBlock Origin}. uBlock Origin introduced new filter types \texttt{queryprune} in October 2020 and then \texttt{removeparam} \cite{ublock-queryprune-github}.
%
Unlike AdGuard, uBlock Origin supports regular expression-based filters to remove tracking query parameters. 
%
At the time of writing, uBlock Origin includes 46 query parameter rules \cite{github-ublock-assets}.

%%
Similar to filter lists used by browsers, these filter lists also suffer from the same issues of manual curation, accuracy, and speed of update.

\subsubsection{Countermeasures proposed by prior research}
To address the issues faced by countermeasures deployed by browsers and extensions, Randall \etal \cite{randall2022measuring} proposed CrumbCruncher -- a semi-automated approach to detect query parameters involved in the exfiltration of identifiers.
%
CrumbCruncher conducts parallel and consecutive crawls to identify query parameters that are distinct across parallel crawls but persistent across consecutive crawls.  
%%we manually removed 577 out of 
%
However, their approach is susceptible to false positives and false negatives. 


%%
Specifically, not all persistent parameters are predisposed to be tracking, e.g., parameters such as \texttt{share\_button} or \texttt{en-US} which remain consistent during multiple visits by the same user, however, they are not used for tracking.
%
This is evidenced by the manual review by the authors, where they identify more than 36\% of the detected identifiers as false positives.
%
% Using CrumbCruncher, the authors shortlisted 1,581 query parameters. 
%
% However, since this shortlist of query parameters contains a large number of false positives, they manually vet it to detect and eliminate more than 36\% false positives to identify about one thousand tracking query parameters. 
%
% In addition to eliminating false positive with manual vetting, 
%
CrumbCruncher also suffers from false negatives because it incorrectly assumes that tracking query parameters are persistent across subsequent crawls.
%
We find that almost 80\% of potential identifiers (i.e., longer than 8 characters as defined by CrumbCruncher) that are exfiltrated to known tracking endpoints (defined using EasyList \cite{easylist} and EasyPrivacy \cite{easyprivacy}) via query parameters change their value across consecutive crawls. % 
%
For example, the \texttt{\_gid} query parameter, which is used by Google Analytics to send a unique user identifier \cite{googlegidparameterdoc}, does not keep a consistent value across consecutive crawls in the same sessions in most of the cases. 
%
As another example, the \texttt{fbp} query parameter, which is used by Meta Pixel to share user identifiers stored in the \texttt{\_fbp} cookie, does not maintain its value in about 87\% of the cases.\footnote{Bekos \etal \cite{bekos2023hitchhiker} showed that the value of the \texttt{\_fbp} cookie (and consequently the \texttt{fbp} query parameter) is randomly chosen from a list of up to 50 different identifiers, resulting in a new identifier for the same user each time.}
%
In summary, CrumbCruncher suffers from non-trivial false positives and false negatives due to its simplistic definition of what constitutes an identifier.
%
In \name, we address this limitation by comprehensively modeling the behavior of link decorations to identify distinguishing characteristics of tracking link decorations.



==> graveyard/breakage_analysis_old.tex <==
\Ht{
This is divided into two parts:

\begin{itemize}
    \item \textbf{Evaluation of primitive techniques to restrict query parameters.}
    \item \textbf{Evaluation of sophisticated countermeasures to restrict query parameters}
\end{itemize}

\para{Primitive Techniques}.

Evaluation of breakage that occurs when we use following configurations to limit query parameters:
\begin{itemize}
    \item Block all query parameters
    \item Blocking all query parameters from third-party requests
    \item Block query parameters from third-party requests not labelled by easyprivacy and easylist
    \item Impact of replacing query parameters instead of blocking
\end{itemize}

\para{Evaluation of sophisticated techniques}

Evaluation of breakage that occurs when following sophisticated countermeasures are used:

\begin{itemize}
    \item UID smuggling paper approach
    \item EasyPrivacy and EasyList
    \item CookieGraph (block query parameters exfiltrating only cookiegraph labelled cookies)
    \item \name
\end{itemize}
}

In this section, we examine different query parameter sanitization methods to gain a more thorough understanding of their effect on user experience during site navigation.
%
These sanitization methods are categorized into primitive and sophisticated techniques to find and "sanitize" query parameters.
%\hl{should I define sanitize}
%
Before examining these methods, however, we will define how we calculate page breakage.

\para{Primitive Techniques of Query Parameter Sanitization} 
%\hl{what makes something a primitive technique?}
%
First for query parameter sanitization are techniques that use generic rules to manipulate request URLs and change query parameters.
%
Individuals may ask the need for advanced sanitization methods; what is the downside of just removing all query parameters? 
%
To respond to this concern, we provide the following analysis for page breakage when applying the four primitive sanitization techniques:
%\hl{why these four?}


\begin{itemize}
    \item Removing all query parameters from all requests
    \item Removing all query parameters from all third-party requests
    \item Removing all query parameters from third-party-requests which EasyList\cite{easylist} and EasyPrivacy\cite{easyprivacy} do not label.
    \item Replacing all query parameters values from third-party requests by replacing each character in the value with a character of the same type (letter with a letter, number for a number).
\end{itemize}

In total we crawled 10k sites. Of those 10k sites, 7287 observed sites crawled successfully and captured a screenshot. We found the number of sites experiencing breakage to be: when blocking all requests to be 804, , blocking third party 441, ?, ? respectively to the listed sanitization methods...
%
\Ht{insert breakage analysis here}

% plan to insert figures here of the four different bing images when I learn how to insert figures and if it is what I should do
% how many examples should I give, since this only shows why blocking all query parameters is bad, do i include an example where third party is broken as well
A manual review of sites exhibiting a high p-hash distance reveal several different cases of primitive query parameter sanitization negatively impacting a sites performance. % find better word for performance
%
Figures 1, 2, 3, and 4 display the homepage of the search engine Bing under different levels of sanitization.
%
Figure 1 is the unchanged site without any sanitization.
%
We can observe that figure 2, blocking all query parameters, is the most different from the others, failing to load most of the content of the page as well as background image.
% would we call this breakage
Figure 3, blocking third party parameters, is more subtle in its differences, as it doesn't display the top stories or weather section at the bottom of the page like in figure 1.
% whether or not this constitutes breakage, is ...
In figure 4, replacement of third party parameters, we can see a new section for the "Image of the day" appear at the bottom of the screen as the viewport of the page appears faulty.
%
From this example of Bing, we can tell that the blocking of all query parameters is unviable, resulting in definite breakage of at least some popular sites.

\para{Sophisticated Techniques of Query Parameter Sanitization}

==> graveyard/decoration-parties.tex <==
\begin{table}[]
    \centering
    \caption{Top }
    \begin{tabular}{c c}
    \toprule
           \textbf{Source} & \textbf{Destination} \\
    \midrule
                  Adform &         Google \\
    googletagmanager.com &         Google \\
                 Raptive & RubiconProject \\
               BidSwitch &         Google \\
                 Raptive &          OpenX \\
                 Raptive &         Yahoo! \\
                  Yahoo! &         Google \\
                DynAdmic &         Google \\
          The Trade Desk &          Tapad \\
               Simpli.fi &         Google \\
            StackAdapt &         Google \\
          The Trade Desk &         Google \\
                  Google &      BidSwitch \\
                 Zemanta &         Google \\
        ClickCertain &         Google \\
                  DataXu &         Google \\
             Rocket Fuel &         Google \\
           IndexExchange &         Google \\
               Quantcast &         Google \\
                   Adobe &         Google \\
    \bottomrule
    \end{tabular}
    \label{tab:my_label}
\end{table}

==> graveyard/decoration-source-destination-entities.tex <==
\begin{table}[htpb]
	\centering
\resizebox{\linewidth}{!}{	
 \begin{tabular}{l c c r}
		\toprule
		\textbf{Link}       & \textbf{Source}       & \textbf{Destination}  & \textbf{Percentage} \\
		\textbf{Decoration} & \textbf{Organization} & \textbf{Organization} & \textbf{of Sites}   \\
		\midrule
	cid                          & Google          & Google              & 62.34      \\
	\_gid                        & Google          & Google              & 41.93      \\
	cookie                       & Google          & Google              & 16.39      \\
	gpic                         & Google          & Google              & 16.35      \\
	auid                         & Google          & Google              & 11.21      \\
	fbp                          & Facebook        & Facebook            & 10.54      \\
	ga\_vid                      & Google          & Google              & 9.98       \\
	DotomiTest                   & ConversantMedia & ConversantMedia     & 7.90       \\
	random                       & Google          & Google              & 5.83       \\
	ga\_sid                      & Google          & Google              & 5.74       \\
	dt                           & Google          & Google              & 5.26       \\
	lmt                          & Google          & Google              & 4.35       \\
	fst                          & Google          & Google              & 4.19       \\
	google\_hm                   & Google          & Google              & 3.99       \\
	rst                          & Google          & Google              & 3.84       \\
	sid                          & Google          & Google              & 3.78       \\
	google\_hm                   & Adform          & Google              & 3.34       \\
	google\_hm                   & IndexExchange   & Google              & 3.27       \\
	sid                          & Microsoft       & Microsoft           & 2.97       \\
	vid                          & Microsoft       & Microsoft           & 2.97       \\
	partner\_device\_id          & The Trade Desk  & Tapad               & 2.92       \\
	ts                           & Facebook        & Facebook            & 2.90       \\
	it                           & Facebook        & Facebook            & 2.65       \\
	khaos                        & RubiconProject  & RubiconProject      & 2.64       \\
	external\_user\_id           & 33Across        & 33Across            & 2.64       \\
	dl                           & Google          & Google              & 2.64       \\
	google\_hm                   & BidSwitch       & Google              & 2.62       \\
	p                            & PubMatic        & PubMatic            & 2.51       \\
	piggybackCookie              & Simpli.fi       & PubMatic            & 2.50       \\
	dlt                          & Google          & Google              & 2.32       \\
	ttd\_puid                    & The Trade Desk  & Tapad               & 2.30       \\
	ref                          & Google          & Google              & 2.24       \\
	ts                           & 33Across        & 33Across            & 2.19       \\
	url                          & Google          & Google              & 2.18       \\
	domain                       & Google          & Google              & 1.94       \\
	google\_hm                   & Yahoo!          & Google              & 1.93       \\
	prevuid                      & DynAdmic        & DynAdmic            & 1.87       \\
	google\_hm                   & OpenX           & Google              & 1.86       \\
	ttd\_puid                    & Tapad           & The Trade Desk      & 1.76       \\
	bidder\_uuid                 & LiveIntent      & LiveIntent          & 1.75       \\
	userId                       & FreeWheel       & FreeWheel           & 1.72       \\
	info                         & Criteo          & Criteo              & 1.69       \\
	google\_hm                   & FreeWheel       & Google              & 1.67       \\
	puid                         & LiveIntent      & Merkle              & 1.67       \\
	google\_push                 & BidSwitch       & Google              & 1.64       \\
	uvs                          & AddThis         & AddThis             & 1.63       \\
	google\_hm                   & RubiconProject  & Google              & 1.62       \\
	id                           & RubiconProject  & Amazon.com          & 1.61       \\
	external\_user\_id           & AT\&T           & IndexExchange       & 1.60       \\
	pr-bh.ybp.yahoo.com$|$path$|$2 & Yahoo!          & Yahoo!              & 1.55       \\
 \bottomrule
\end{tabular}
}
\caption{Top-50 ATS link decorations and their source and destination organizations}
	\label{tab:decoration-source-destination-entities}
\end{table}

==> graveyard/feature-importance-negative.tex <==
\begin{table}[]
    \centering
     \caption{Percentage of instances where a feature was most important for \nonats link decorations}
    \begin{tabular}{l c}
    \toprule
    \textbf{Feature}   & \textbf{Percentage}  \\
    \midrule
    Closeness Centrality of Indirect Edges  &         55.24\% \\
    Out Degree of Indirect Edges             &        28.61\% \\
    Number of Exfiltrations                       &        13.14\% \\
    Number of Indirect Descendents             &        1.69\% \\
    Shannon Entropy                  &        0.51\% \\
    Number of Indirect Ancestors               &        0.43\% \\
    In Degree of Indirect Edges                &        0.2\% \\
    Average Connectivity of Indirect Edges &     0.1\% \\
    In Degree                        &        0.03\% \\
    Presence of AD Keyword in Ascendent        &         0.01\% \\
    \bottomrule
    \end{tabular}
   
    \label{tab:feature-importance-negative}
\end{table}

==> graveyard/feature-importance-overall.tex <==
\begin{table}
    \centering
    \caption{Top 10 most important features}
    \begin{tabular}{l c}
    \toprule
    Feature    & Importance \\
    \midrule
    indirect\_closeness\_centrality      &         0.1422 \\
    num\_exfil                          &        0.1326 \\ 
    indirect\_out\_degree                &         0.1249 \\
    indirect\_descendants               &         0.1214 \\ 
    indirect\_ancestors                  &        0.1158 \\
    indirect\_average\_degree\_connectivity &       0.1152 \\
    indirect\_in\_degree                 &         0.1044 \\
    shannon\_entropy                   &          0.0331 \\
    max\_depth\_decoration             &           0.0163 \\
    indirect\_all\_in\_degree           &           0.0138 \\
    indirect\_all\_ancestors           &           0.0131 \\
    \bottomrule
    \end{tabular}
    \label{tab:feature-importance-overall}
\end{table}

==> graveyard/intro_old.tex <==


Privacy-preserving tools (browsers, content blockers, etc.) and trackers have been up at arms against each other since the advent of online advertising \cite{easylist, easyprivacy, JohnWebkit2017ITP, firefox-etp, ublock-cookie-remover} \Ht{conflating advertising and tracking} .
%
Where blocking of third-party cookies dealt a significant blow to an obvious and easy way to track users across sites \cite{JohnWebkit2019ITP-2-2, GooglePrivacySandbox, firefox-cookie-policy}, it is no secret that trackers are actively looking to compensate for the loss of third-party cookies with new ways to track users by repurposing web resources used for functional usage into tracking.
\Ht{informal.. rephrase} 
%
Examples of such resources include first-party cookies \cite{FranziskaUSENIX12, Fouad20PixelsPETS, ChenACM2021CookieSwapParty, Munir23CookieGraphArxiv}, first-party data including emails, phone numbers, etc. \cite{cartologychang2022ccs}, and fingerprinting using information such as IP addresses \cite{?}, hardware specification \cite{?}, etc.
\Ht{I don't believe IP address based tracking is relevant to our work.} 


% %%
A common theme among the use of all these different resources is that information collected through these sources is sent by trackers to their own servers.
%
Trackers make use of HTTP Requests API for this purpose.
\Ht{Why mention "API"? AFAIK non-script initiated requests don't use the API. Let's keep it generic?}
%
HTTP Requests API allows tracking resources such as scripts, pixels, images, etc., to contact an endpoint on their own servers.
%
Trackers can append additional information about users, which can contain first-party  cookie values or fingerprints, to these requests by making use of link decorations.
\Ht{Trackers don't append to "requests", they append to "hyperlinks/links" in the requests. Right? If so, please rephrase}



Link decorations are query parameters, resource paths, and fragments appended to a URL.
%
While there are functional uses of link decorations, examples of which include but are not limited to: identifying a product while navigating an online store, using CSRF (Cross-Site Request Forgery) tokens to protect against request vulnerabilities, and authenticating through SSO (single-sign-on) services \Ht{add citations to these functional use cases if possible}, their use for tracking purposes is becoming more common. 
%
Thus to effectively counter tracking through new avenues in absence of third-party cookies \Ht{why emphasis on 3P cookies all of the sudden?}, it is pertinent to restrict the unchecked use \Ht{colloquial language} of link decoration by advertisers and trackers. \Ht{again, conflating advertising and tracking}



%%
In addition to extensive use of link decoration in purely tracking requests, functional requests are also decorated with additional information which can be used for identifying user activity.\Ht{This is an important point but doesn't flow well. It needs to be motivated and perhaps needs to go with the previous paragraph.}
%
To prevent this, many privacy-focused browsers (Firefox, Brave, \Ht{Safari too?}) and extensions (uBlock Origin, AdGuard) have started including lists of known query parameters that are appended to URLs for tracking purposes.
%
While this approach might work for a smaller number of well-known tracking query parameters, it cannot keep pace with the adoption of link decoration by trackers.\Ht{can we provide citation or justify this implicit claim that adoption of link decoration is increasing?}
%
In addition to this, existing countermeasures and research does not take into account link decoration techniques other than query parameters.\Ht{Important point but we need to say more. Can we say that trackers have started to exploit path or fragments because they are aware that query parameters are stripped/sanitized?}
%
In this paper, we show that link decoration by trackers is not limited to only query parameters, but resource paths and fragments are also used to relay information about the user for tracking purposes.


%%
\Ht{this para needs to be rewritten in light of our new measurement section}
We perform a measurement study on 20K websites and show that link decoration is widely used by trackers, with ?\% of websites sending HTTP requests with potentially identifiable information in link decorations, while 3.78\% of sites found sending personal information such as email in link decorations.
%
Our analysis also reveals that link decoration is widely used in cookie-syncing, which is a popular way for trackers to collude with each other \cite{?}.
%
Our measurements find that 69.39\% of sites share advertising and tracking cookie values through link decorations.
%
Our research also shows that existing countermeasures are not enough to prevent tracking through link decorations.
%
These countermeasures either rely on very limited lists of tracking query parameters (FireFox, Brave, uBlock Origin, AdGuard), or their definition of tracking link decorations is limited only to a smaller subset of potential privacy invasive decorations \cite{UIDSmugglingPaper}.


%%
We propose \name (pronounced Purell), a machine learning-based approach to automatically detect tracking link decorations.
%
\name captures fundamental tracking behaviors associated with link decorations to accurately and robustly identify \ats decorations in request URLs.
%
Our analysis shows that \name outperforms existing countermeasures by at least 8\%, and reduces major website breakage caused by these countermeasures by ?\%.
%
\Ht{quantify robustness}
\Ht{cite related work it outperforms}


%%
We deploy \name on 20K websites to find \ats link decorations on 68.95\% of sites.
%
We show that the most prevalent \ats link decorations are used by well-known advertising/tracking entities such as Google, Facebook, and Microsoft.
%
We find that ?\% of \ats link decorations exfiltrate values stored in first-party tracking cookies, while ?\% of link decorations are used by scripts involved in fingerprinting.



%%
In summary, our key contributions are:

\begin{enumerate}
    \item We conduct a measurement study on 20K websites, showing the large-scale use of link decorations by trackers. Our analysis shows that it is not trivial to remove tracking link decorations as either the list of known tracking decorations is limited, the methodology to automatically detect tracking link decorations is unable to capture all tracking instances of link decorations, and the removal of all link decorations results in significant website-breakage.
    \item We propose \name, a machine learning-based approach to automatically detect tracking link decorations. We show that \name outperforms existing countermeasures in accuracy, robustness, and minimization of website breakage.
    \item We deploy \name on 20K websites to measure the prevalence of tracking link decorations. We detect a total of ? tracking domains making use of link decorations to exfiltrate identifiable information about users, including information in browser storage and emails entered on the webpage.
\end{enumerate}

==> graveyard/link-decoration-stats.tex <==
\begin{table}[]
  \centering
  \caption{Caption\Ht{write a caption; do we really need this table? it's covered in first para of 3.2, no?}}
  \resizebox{\linewidth}{!}{
    \begin{tabular}{l c c c}
      \toprule
      {}                      & \textbf{Resource Paths} & \textbf{Query Parameters } & \textbf{Fragments} \\
      \midrule
      Total Link Decorations  & 18,672,132              & 25,959,949                 & 11,625             \\
      Unique Link Decorations & 314,582                 & 267,714                    & 1,473              \\
      \bottomrule
    \end{tabular}
  }
  \label{tab:link-decoration-stats}
\end{table}

==> graveyard/linkdecoration-email-domain-first-party-top-10.tex <==
\begin{table}[]
    \centering
    \caption{Top 10 Domains With Emails In Link Decorations In Requests To First Party Sites}
    \begin{tabular}{l c}
        \toprule
        Domain     &   Instances \\
        \midrule
        pinterest.com                       & 49  \\
        tomas.com                           & 44  \\
        domotz.com                          & 12  \\
        paydayloansonlinedirect.com         & 9   \\
        brides.com                          & 9   \\
        secretescapes.com                   & 9   \\
        zapier.com                          & 8   \\
        travelportland.com                  & 8   \\
        wwt.com                             & 6   \\

        \bottomrule
    \end{tabular}
    \label{tab:linkdecoration-email-domain-first-party-top-10}
\end{table}

==> graveyard/linkdecoration-email-domain-third-party-top-10.tex <==
\begin{table}[]
    \centering
    \caption{Top 10 domains which receive emails in link decorations}
    \begin{tabular}{l c}
        \toprule
        \textbf{Domain}     &   \textbf{Organization} \\
        \midrule
        list-manage.com                     & Mailchimp  \\
        listrakbi.com                       & Listrak  \\
        shop.com                            & SHOP.COM  \\
        google-analytics.com                & Google   \\
        evergage.com                        & SalesForce   \\
        heapanalytics.com                   & Heap   \\
        getvero.com                         & Vero   \\
        lfeeder.com                         & Leadfeeder   \\
        doubleclick.com                     & Google   \\
        terminus.com                        & Terminus   \\
        \bottomrule
    \end{tabular}
    \label{tab:linkdecoration-email-domain-third-party-top-10}
\end{table}

==> graveyard/linkdecoration-email-key-top-10.tex <==
\begin{table}[]
    \centering
    \caption{Top 10 Link Decoration Keys Used when Passing Email Values }
    \begin{tabular}{l c}
        \toprule
        Query Parmeter Key &   Instances \\
        \midrule
        email        & 263  \\
        data         & 63  \\
        EMAIL        & 61  \\
        term         & 44  \\
        username     & 15  \\
        info         & 13   \\
        k\_0          & 10   \\
        event        & 9   \\
        params       & 9   \\
        value        & 8   \\
        \bottomrule
    \end{tabular}
    \label{tab:linkdecoration-email-key-top-10}
\end{table}

==> graveyard/methodology.tex <==
%In this section, we define link decoration and describe different types of link decorations.


%%
\subsection{URL Structure}
A URL is composed of several segments, including a scheme, a fully qualified domain name (FQDN), a resource path, recourse name, query parameters, and fragments.
%
We use \textcolor{blue}{https}://\textcolor{green}{example.com}/\textcolor{violet}{YYY/ZZZ/}\textcolor{magenta}{pixel.jpg}?\textcolor{red}{ISBN=XXX \&UID=ABC123}\#\textcolor{orange}{xyz}, as an example URL to define these segments, below:

% Below, we define different parts of the URL using the following example: \textcolor{blue}{https}://\textcolor{green}{example.com}/\textcolor{violet}{YYY/ZZZ/pixel.jpg}?\textcolor{red}{ISBN=XXX \&UID=ABC123}\#\textcolor{orange}{xyz}.


\para{Base URL}. \textcolor{blue}{https://} is the scheme in this URL and \textcolor{green}{example.com} is the FQDN. These segments are combined to form the base URL.  


\para{Resource path}. \textcolor{violet}{YYY/ZZZ} is the resource path in the URL, corresponding to the directory path on the server, and \textcolor{magenta}{pixel.jpg} is the resource name hosted on the server. 
%
The resource path immediately follows the FQDN.


\para{Query parameters}. \textcolor{red}{ISBN=XXX\&UID=abc123} are the query parameters in the URL. 
%
A query parameter consists of a key-value pair, where the key is separated from the value by the = delimiter.
%
Multiple query parameters in a URL are separated by the \& delimiter.
%
The query parameters immediately follow the resource path and are separated by the ? delimiter.


\para{Fragments}. \textcolor{orange}{xyz} is the fragment in the URL. 
%
Fragments can be a singular value or multiple key-value pairs that are separated by the \& delimiter (similar to query parameters).
%
The fragments immediately follow the query parameter and are separated by the \# delimiter.




\subsection{Link Decoration: Abuse of URL segments for tracking}
URL query parameters and fragments have been abused for tracking as early as the inception of the web.
%
For example, \textit{Webtrends}, an analytics service used the \textit{WT.mc\_id} query parameter to track clicks and site visits across multiple marketing campaigns\cite{webtrends1996} in 1996.
%
% In recent years, thanks to the omnipresent online tracking and advertising services, web users are constantly targeted for their personal information - often without their explicit consent. 
%
\xxx[Umar]{Here we should discuss some of the recent instances or anecdotal evidence of the use of URL segments for tracking. Including AdTech docs which recommend or use link decoration. I have also copied the discussion of URL smuggling paper below (from ``adoption of link decoration'' subsection) but it needs to be revised.}
%
In recent years, URL decoration, as a means of tracking, has become a favorable choice for trackers due to its ease of use compared to cookies or fingerprinting, which require additional handling and setup on the client and server sides. 
%
One such case is the UID \textit{smuggling} \cite{randall2022measuring}, which is an emerging tracking technique geared towards evading current privacy protections. 
%
UID \textit{smuggling} works by inserting user identifiers (UIDs) in a user's web navigation request. 
%
This allows trackers to synchronize UIDs and, hence, gain the ability to track users across sites. 
%
Although this paper, by Randal et al., conjectures that UIDs for individual users remain the same across sites, as will be shown in this work, for instance, the \texttt{fbp} identifier is chosen randomly from 50 identifiers and changes for the same user again and again.



%%
\subsection{Link Decoration}
At a high level, link decoration is everything except for the base URL. 
%
More precisely, link decoration includes resource path (excluding the file name), query parameters, and fragments.


\para{Naming Link Decorations.}
To track link decoration across different URLs, we need a consistent naming scheme that is able to identify individual link decorations.
%
When link decorations are in the key-value format, the key can simply be combined with FQDN\footnote{We consider FQDN because the standards/specs only define the format but not the name of the link decorations. A server can arbitrarily name its own keys.} to uniquely identify a link decoration.
%
When link decorations are not in key-value format (resource path and singular value fragments), we assign them keys based on the FQDN and their position in the URL.
%
For resource paths, we consider different directory levels separately and identify them based on their distance from the root. 
%
For the aforementioned example URL, we identify the following link decorations:
%%

\begin{enumerate}
    \item example.com$|$path$|$1: YYY
    \item example.com$|$path$|$2: ZZZ
    \item example.com$|$ISBN: XXX
    \item example.com$|$UID: ABC123
    \item example.com$|$fragment: xyz
\end{enumerate}


This naming scheme allows us to compare link decoration values across different URLs.




%We use the terminology of link decoration as defined in Privacy Community Group's report \cite{link-decoration-privacycg}. 
% According to this definition, link decoration is any addition of information to a URL that extends beyond what is required to identify a webpage.
% %
% Link decoration can further be categorized into three different types based on their usage, deliminator, and location in the URL: query parameters, path parameters, and fragments.
%%




%For fragments which contain multiple key-value pairs, we consider each key-value pair individually in our analysis.


% For example, if the URL's purpose is to redirect the user to a book with a particular ISBN on click, any information added to the URL apart from the book ISBN can be characterized as link decoration.
% %
% In case of a sample URL, \texttt{https://example.com/abcdefgh/?ISBN=XXXXXXXXXXXX\&UID=\\abc123\#xyz}, the addition of \texttt{UID} is considered link decoration.

% Link Decoration can further be categorized into following different types:

% \para{Query Parameter}. We define query parameter as a key value pair added to a URL. A query paramter can be used for both functional as well as tracking purposes.
% %
% For example, in the example described earlier, \texttt{ISBN} is an example of a functional query parameter, while \texttt{UID} is an example of a tracking query parameter.
% %%

% \para{Path Parameter}. We define the URL path parameters as ``\textbackslash'' separated parameters between the eTLD+1 domain and the query parameters.

% For example, in the earlier example, \texttt{abcdefgh} is an example of a URL path parameter.

% \para{Fragment}. We define a fragment as an appendage to the URL after the query parameters, preceded by ``\#''. Fragments are commonly as an identifier to a CSS section within the website page.

% For example, \texttt{xyz} is a fragment in the earlier example.\Ht{Replace with real examples}


% We now describe threat model to explain how user tracking is enabled through query parameters. 
% \Ht{There can be following different threat models:

% \begin{itemize}
%     \item \textbf{Exfiltration of information out of the webpage}. User visits a site, information about the user is collected (email addresses, fingerprints etc.). The information is sent through query parameters, the tracking server takes in the information and returns an identifier of the user. Upon subsequent visits of the user, the same identifier is sent through query parameters. In this model, the script collecting information and the server sending back the identifier all belong to third-parties, potentially running in a first-party context. With no additional tracking information available from any other source, this technique works as well as the collected data, i.e. if the data collected can be coalesced to determine user identity on a large number of sites, it can be used to track user across sites. However, if the data collection is primitive, the information can only be used for same-site tracking.
%     \item \textbf{Infiltration of information into the webpage}. The second case is where information from outside the webpage is sent to the webpage to help it determine user identity. For example, the user clicks a link on Facebook to lead towards another site example.com. Facebook appends additional information to the link which is read by the site and that information can be used to identify user. In this case, the user need not have visited the site and can be identified across different sites.
%     {This can be merged and explained with case studies instead}
% \end{itemize}
% }

==> graveyard/queryparam-label-cookiegraph-top-10.tex <==
\begin{table}[]
	\centering
	\begin{tabular}{l c c}
		\toprule
		Cookie          & Query Parameter & Instances \\
		\midrule
		\_ga            & cid             & 271865    \\
		\_\_gpi         & gpic            & 79013     \\
		\_ga            & ga\_vid         & 58986     \\
		\_\_gads        & cookie          & 56036     \\
		\_gid           & \_gid           & 47620     \\
		\_fbp           & fbp             & 34916     \\
		\_gcl\_au       & auid            & 33315     \\
		\_\_hssc        & b               & 30588     \\
		cto\_bundle     & bundle          & 17639     \\
		\_\_adroll\_fpc & adroll\_fpc     & 15770     \\
		\bottomrule
	\end{tabular}
	\caption{Top 10 Tracking Cookies labelled by CookieGraph and their Query Parameter Pairs}
	\label{tab:queryparam-label-cookiegraph-top-10}
\end{table}

==> graveyard/queryparam-label-cookiepedia-top-10.tex <==
\begin{table}[htpb]
	\centering
	\begin{tabular}{l c r}
		\toprule
		\textbf{Storage Key} & \textbf{Link Decoration} & \textbf{Sites} \\
		\midrule
		\_ga            & cid                      & 11,351              \\
		\_gid           & \_gid                    & 4,843               \\
		\_fbp           & fbp                      & 3,784               \\
		\_ga            & ga\_vid                  & 2,015               \\
		\_\_gads        & cookie                   & 1,306               \\
		CN\_sp          & uID                      & 1,131               \\
		\_\_hssc        & b                        & 992                \\
		CN\_xid         & xID                      & 882                \\
		\_uetsid        & sid                      & 692                \\
		\_gcl\_au       & auid                     & 627                \\
		\bottomrule
	\end{tabular}
	\label{tab:queryparam-label-cookiepedia-top-10}
 \vspace{-10pt}
 	\caption{Top-10 \ats storage keys exfiltrated through \ats link decorations}
  \vspace{-10pt}
\end{table}

==> graveyard/top-100-link-decorations-sources-destinations.tex <==
\begin{table}[htpb]
  \centering
  \resizebox{\linewidth}{!}{\begin{tabular}{l c c r}
      \toprule
      \textbf{Link}                           & \textbf{Source}       & \textbf{Destination} &
      \textbf{\%}                                                                      \\
      \textbf{Decoration}                     & \textbf{Domain}       & \textbf{Domain}      &
      \textbf{of Sites}                                                                        \\
      \midrule
      google\_hm                              & smartadserver.com     &
      doubleclick.net                         & 1.46                                           \\
      google\_hm                              & pubmatic.com          &
      doubleclick.net                         & 1.43                                           \\
      google\_hm                              & lijit.com             &
      doubleclick.net                         & 1.43                                           \\
      cid                                     & doubleclick.net       &
      google.com                              & 1.40                                           \\
      piggybackCookie                         & simpli.fi             &
      pubmatic.com                            & 1.40                                           \\
      partner\_device\_id                     & adnxs.com             &
      tapad.com                               & 1.39                                           \\
      bundle                                  & criteo.com            &
      criteo.com                              & 1.39                                           \\
      put                                     & adsrvr.org            &
      rubiconproject.com                      & 1.35                                           \\
      prevuid                                 & dyntrk.com            &
      dyntrk.com                              & 1.34                                           \\
      google\_hm                              & teads.tv              &
      doubleclick.net                         & 1.33                                           \\
      ts                                      & 33across.com          &
      33across.com                            & 1.32                                           \\
      google\_push                            & bidswitch.net         &
      doubleclick.net                         & 1.32                                           \\
      anx\_uId                                & adnxs.com             &
      clickcertain.com                        & 1.31                                           \\
      i                                       & openx.net             &
      gumgum.com                              & 1.31                                           \\
      google\_push                            & googlesyndication.com &
      doubleclick.net                         & 1.31                                           \\
      cookie                                  & doubleclick.net       &
      doubleclick.net                         & 1.31                                           \\
      gpic                                    & doubleclick.net       &
      doubleclick.net                         & 1.31                                           \\
      put                                     & adnxs.com             &
      rubiconproject.com                      & 1.29                                           \\
      i                                       & adsrvr.org            &
      gumgum.com                              & 1.28                                           \\
      cookie                                  & 2mdn.net              &
      doubleclick.net                         & 1.27                                           \\
      gpic                                    & 2mdn.net              &
      doubleclick.net                         & 1.27                                           \\
      fbp                                     & facebook.com          &
      facebook.com                            & 1.27                                           \\
      partner\_device\_id                     & crwdcntrl.net         &
      tapad.com                               & 1.26                                           \\
      piggybackCookie                         & adsrvr.org            &
      pubmatic.com                            & 1.26                                           \\
      i                                       & yahoo.com             &
      gumgum.com                              & 1.24                                           \\
      ruxId                                   & rubiconproject.com    &
      linkedin.com                            & 1.24                                           \\
      google\_push                            & googlesyndication.com &
      bidswitch.net                           & 1.24                                           \\
      i                                       & adnxs.com             &
      gumgum.com                              & 1.23                                           \\
      khaos                                   & rubiconproject.com    &
      rubiconproject.com                      & 1.23                                           \\
      google\_hm                              & adnxs.com             &
      doubleclick.net                         & 1.23                                           \\
      piggybackCookie                         & adnxs.com             &
      pubmatic.com                            & 1.22                                           \\
      i                                       & bidswitch.net         &
      gumgum.com                              & 1.22                                           \\
      prevuid                                 & googlesyndication.com &
      dyntrk.com                              & 1.21                                           \\
      DotomiTest                              & dotomi.com            &
      dotomi.com                              & 1.21                                           \\
      i                                       & mathtag.com           &
      gumgum.com                              & 1.21                                           \\
      i                                       & everesttech.net       &
      gumgum.com                              & 1.21                                           \\
      partner\_uid                            & openx.net             &
      rlcdn.com                               & 1.20                                           \\
      ga\_vid                                 & 2mdn.net              &
      doubleclick.net                         & 1.19                                           \\
      i                                       & qvdt3feo.com          &
      gumgum.com                              & 1.19                                           \\
      uid                                     & owneriq.net           &
      owneriq.net                             & 1.18                                           \\
      google\_hm                              & simpli.fi             &
      doubleclick.net                         & 1.18                                           \\
      anx\_uId                                & googlesyndication.com &
      clickcertain.com                        & 1.18                                           \\
      ttd\_tdid                               & adsrvr.org            &
      doubleclick.net                         & 1.17                                           \\
      user\_id                                & mookie1.com           &
      bidswitch.net                           & 1.17                                           \\
      put                                     & simpli.fi             &
      rubiconproject.com                      & 1.17                                           \\
      i                                       & ipredictive.com       &
      gumgum.com                              & 1.17                                           \\
      sync.targeting.unrulymedia.com||path||1 & 1rx.io                &
      unrulymedia.com                         & 1.17                                           \\
      ns\_\_t                                 & scorecardresearch.com &
      scorecardresearch.com                   & 1.17                                           \\
      i                                       & outbrain.com          &
      gumgum.com                              & 1.17                                           \\
      bidder\_uuid                            & liadm.com             &
      liadm.com                               & 1.15                                           \\
      \bottomrule
    \end{tabular}
  }

  \caption{Top-100 \ats link decorations, their source and destination domains
    based on their prevalence on 20K sites}
  \label{tab:top-100-link-decorations-sources-destinations}
\end{table}

==> graveyard/top-20-decorations-destination.tex <==
\begin{table}[]
	\centering
	\caption{Top-20 \ats link decorations and their destinations based on their prevalence on 20K sites}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{l c c c}
			\toprule
			\textbf{Link}       & \textbf{Destination} & \textbf{Organization}   & \textbf{Percentage} \\
			\textbf{Decoration} & \textbf{Domain}      & \textbf{}               & \textbf{of Sites}   \\
			\midrule
			cid                 & google-analytics.com & Google              & 45.90               \\
			\_gid               & google-analytics.com & Google              & 41.77               \\
			cid                 & doubleclick.net      & Google              & 29.57               \\
			\_gid               & doubleclick.net      & Google              & 27.93               \\
			cid                 & google.com           & Google              & 22.25               \\
			fbp                 & facebook.com         & Facebook          & 19.98               \\
			cookie              & doubleclick.net      & Google              & 12.53               \\
			gpic                & doubleclick.net      & Google              & 12.51               \\
			auid                & doubleclick.net      & Google              & 10.44               \\
			ga\_vid             & doubleclick.net      & Google              & 10.14               \\
			vid                 & bing.com             & Microsoft   & 5.81                \\
			sid                 & bing.com             & Microsoft   & 5.80                \\
			cookie              & googleadservices.com & Google              & 5.46                \\
			gpic                & googleadservices.com & Google              & 5.45                \\
			user\_id            & bidswitch.net        & BidSwitch               & 4.78                \\
			partner\_device\_id & tapad.com            & Tapad             & 4.68                \\
			partner\_uid        & rlcdn.com            & LiveRamp & 4.62                \\
			google\_hm          & doubleclick.net      & Google              & 4.47                \\
			id                  & bluekai.com          & Oracle      & 4.31                \\
			uid                 & yahoo.com            & Yahoo!                  & 4.27                \\
			\bottomrule
		\end{tabular}
	}
	\label{tab:top_20_decorations}
\end{table}

==> graveyard/top-50-decorations-destinations.tex <==
\begin{table}[]
	\centering
	\caption{Top-5-0 \ats link decorations and their sources based on their prevalence on 20K sites}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{l c r}
\toprule
          \textbf{Link} &                    \textbf{Domain} &  \textbf{Percentage} \\
          \textbf{Decoration} &                    \textbf{} &  \textbf{of Sites} \\
\midrule
                        cid &       www.google-analytics.com &       56.84 \\
                        \_gid &       www.google-analytics.com &       50.90 \\
                         cid &        stats.g.doubleclick.net &       36.60 \\
                        \_gid &        stats.g.doubleclick.net &       34.04 \\
                         cid &                 www.google.com &       23.43 \\
                         fbp &               www.facebook.com &       19.14 \\
                        auid &    googleads.g.doubleclick.net &       13.41 \\
                         cid &           analytics.google.com &       11.03 \\
                      cookie &    googleads.g.doubleclick.net &        7.72 \\
                        gpic &    googleads.g.doubleclick.net &        7.71 \\
                      ga\_vid &    googleads.g.doubleclick.net &        6.97 \\
                      ga\_vid & securepubads.g.doubleclick.net &        6.69 \\
                      cookie &   partner.googleadservices.com &        5.60 \\
                        gpic &   partner.googleadservices.com &        5.59 \\
                         vid &                   bat.bing.com &        5.55 \\
                         sid &                   bat.bing.com &        5.54 \\
                      cookie & securepubads.g.doubleclick.net &        5.45 \\
                        gpic & securepubads.g.doubleclick.net &        5.42 \\
                         sid &       www.google-analytics.com &        4.99 \\
                     user\_id &                x.bidswitch.net &        4.70 \\
                 partner\_uid &               idsync.rlcdn.com &        4.61 \\
           partner\_device\_id &                pixel.tapad.com &        4.50 \\
                   google\_hm &           cm.g.doubleclick.net &        4.28 \\
                         uid &        ups.analytics.yahoo.com &        4.19 \\
                         put &       pixel.rubiconproject.com &        3.96 \\
                          ts &               www.facebook.com &        3.84 \\
                      ga\_sid & securepubads.g.doubleclick.net &        3.79 \\
                         rst &  pagead2.googlesyndication.com &        3.50 \\
                          it &               www.facebook.com &        3.48 \\
                        auid &                 www.google.com &        3.48 \\
                          id &          s.amazon-adsystem.com &        3.45 \\
                        info &                 gum.criteo.com &        3.30 \\
                         val &                 us-u.openx.net &        3.14 \\
pr-bh.ybp.yahoo.com||path||2 &            pr-bh.ybp.yahoo.com &        3.13 \\
                          dt & securepubads.g.doubleclick.net &        3.12 \\
                          id &               tags.bluekai.com &        3.07 \\
                         fst &    googleads.g.doubleclick.net &        3.05 \\
                      ga\_sid &    googleads.g.doubleclick.net &        2.95 \\
                    ttd\_puid &               match.adsrvr.org &        2.92 \\
                      random &    googleads.g.doubleclick.net &        2.91 \\
                        3pid &                   ce.lijit.com &        2.89 \\
                      random &                 www.google.com &        2.85 \\
            external\_user\_id &       dsum-sec.casalemedia.com &        2.85 \\
                         lmt & securepubads.g.doubleclick.net &        2.77 \\
                        xuid &                  eb2.3lift.com &        2.76 \\
                         sid &           analytics.google.com &        2.71 \\
                         dlt & securepubads.g.doubleclick.net &        2.57 \\
                          dl &       www.google-analytics.com &        2.40 \\
                         lmt &    googleads.g.doubleclick.net &        2.33 \\
                 bidder\_uuid &                    i.liadm.com &        2.30 \\
\bottomrule
\end{tabular}

	}
	\label{tab:top-20-decorations-sources}
\end{table}

==> graveyard/top-50-link-decorations-sources-destinations.tex <==
\begin{table}[htpb]
  \centering
  \resizebox{\linewidth}{!}{ \begin{tabular}{l c c r}
      \toprule
      \textbf{Link}                & \textbf{Source}       & \textbf{Destination}  &
      \textbf{\%}                                                            \\
      \textbf{Decoration}          & \textbf{Domain}       & \textbf{Domain}       &
      \textbf{of Sites}                                                              \\
      \midrule
      cid                          & google-analytics.com  & google-analytics.com  &
      33.75                                                                          \\
      \_gid                        & google-analytics.com  & google-analytics.com  &
      33.54                                                                          \\
      cid                          & googletagmanager.com  & google-analytics.com  &
      12.58                                                                          \\
      fbp                          & facebook.net          & facebook.com          &
      9.27                                                                           \\
      auid                         & googletagmanager.com  & doubleclick.net       &
      7.87                                                                           \\
      cookie                       & googlesyndication.com & googleadservices.com  &
      5.66                                                                           \\
      gpic                         & googlesyndication.com & googleadservices.com  &
      5.65                                                                           \\
      cid                          & google-analytics.com  & doubleclick.net       &
      5.41                                                                           \\
      \_gid                        & google-analytics.com  & doubleclick.net       &
      4.77                                                                           \\
      ga\_vid                      & doubleclick.net       & doubleclick.net       &
      4.50                                                                           \\
      cookie                       & doubleclick.net       & doubleclick.net       &
      4.39                                                                           \\
      gpic                         & doubleclick.net       & doubleclick.net       &
      4.37                                                                           \\
      cid                          & googletagmanager.com  & google.com            &
      4.30                                                                           \\
      google\_hm                   & googlesyndication.com & doubleclick.net       &
      3.88                                                                           \\
      rst                          & googletagservices.com & googlesyndication.com &
      3.75                                                                           \\
      google\_hm                   & adform.net            & doubleclick.net       &
      3.34                                                                           \\
      google\_hm                   & casalemedia.com       & doubleclick.net       &
      3.27                                                                           \\
      ga\_sid                      & doubleclick.net       & doubleclick.net       &
      2.97                                                                           \\
      vid                          & bing.com              & bing.com              &
      2.96                                                                           \\
      sid                          & bing.com              & bing.com              &
      2.96                                                                           \\
      partner\_device\_id          & adsrvr.org            & tapad.com             &
      2.92                                                                           \\
      \_gid                        & googletagmanager.com  & google-analytics.com  &
      2.78                                                                           \\
      cid                          & google-analytics.com  & google.com            &
      2.56                                                                           \\
      ts                           & facebook.net          & facebook.com          &
      2.51                                                                           \\
      dt                           & doubleclick.net       & doubleclick.net       &
      2.47                                                                           \\
      sid                          & googletagmanager.com  & google-analytics.com  &
      2.42                                                                           \\
      cookie                       & googlesyndication.com & doubleclick.net       &
      2.32                                                                           \\
      gpic                         & googlesyndication.com & doubleclick.net       &
      2.32                                                                           \\
      ttd\_puid                    & adsrvr.org            & tapad.com             &
      2.30                                                                           \\
      it                           & facebook.net          & facebook.com          &
      2.30                                                                           \\
      dlt                          & doubleclick.net       & doubleclick.net       &
      2.24                                                                           \\
      random                       & doubleclick.net       & google.com            &
      2.21                                                                           \\
      lmt                          & doubleclick.net       & doubleclick.net       &
      2.13                                                                           \\
      ga\_vid                      & googlesyndication.com & doubleclick.net       &
      2.12                                                                           \\
      google\_hm                   & bidswitch.net         & doubleclick.net       &
      1.96                                                                           \\
      google\_hm                   & yahoo.com             & doubleclick.net       &
      1.92                                                                           \\
      google\_hm                   & openx.net             & doubleclick.net       &
      1.86                                                                           \\
      fst                          & googletagmanager.com  & doubleclick.net       &
      1.84                                                                           \\
      auid                         & googletagmanager.com  & google.com            &
      1.83                                                                           \\
      random                       & googletagmanager.com  & doubleclick.net       &
      1.82                                                                           \\
      ttd\_puid                    & tapad.com             & adsrvr.org            &
      1.76                                                                           \\
      info                         & criteo.com            & criteo.com            &
      1.69                                                                           \\
      puid                         & liadm.com             & rkdms.com             &
      1.67                                                                           \\
      uvs                          & addthis.com           & addthis.com           &
      1.63                                                                           \\
      google\_hm                   & rubiconproject.com    & doubleclick.net       &
      1.62                                                                           \\
      id                           & rubiconproject.com    & amazon-adsystem.com   &
      1.60                                                                           \\
      dl                           & google-analytics.com  & google-analytics.com  &
      1.60                                                                           \\
      pr-bh.ybp.yahoo.com||path||2 & yahoo.com             & yahoo.com             &
      1.52                                                                           \\
      partner\_device\_id          & mathtag.com           & tapad.com             &
      1.49                                                                           \\
      external\_user\_id           & 33across.com          & 33across.com          &
      1.48                                                                           \\
      \bottomrule
    \end{tabular}
  }

  \caption{Top-100 \ats link decorations, their source and destination domains
    based on their prevalence on 20K sites}
  \label{tab:top-50-link-decorations-sources-destinations}
\end{table}

==> graveyard/top_20_decorations_negative.tex <==
\begin{table}[]
	\centering
	\caption{Top-20 \nonats Link Decorations based on their prevalence on 20K sites}
	\resizebox{\linewidth}{!}{
		\begin{tabular}{l c c c}
			\toprule
			\textbf{Link}                          & \textbf{Destination} & \textbf{Organization} & \textbf{Percentage} \\
			\textbf{Decoration}                    & \textbf{Domain}      & \textbf{}             & \textbf{of Sites}   \\
			\midrule
			dl                                     & google-analytics.com & Google LLC            & 59.080              \\
			dt                                     & google-analytics.com & Google LLC            & 56.495              \\
			fonts.gstatic.com$|$path$|$3           & gstatic.com          & Google LLC            & 55.710              \\
			id                                     & googletagmanager.com & Google LLC            & 55.490              \\
			tid                                    & google-analytics.com & Google LLC            & 49.810              \\
			family                                 & googleapis.com       & Google LLC            & 47.185              \\
			www.google.com$|$path$|$1              & google.com           & Google LLC            & 31.370              \\
			tid                                    & doubleclick.net      & Google LLC            & 30.120              \\
			url                                    & doubleclick.net      & Google LLC            & 29.250              \\
			tid                                    & google.com           & Google LLC            & 22.955              \\
			gtm                                    & google-analytics.com & Google LLC            & 21.915              \\
			dr                                     & google-analytics.com & Google LLC            & 20.355              \\
			dl                                     & facebook.com         & Facebook, Inc.        & 19.890              \\
			ref                                    & doubleclick.net      & Google LLC            & 17.910              \\
			googleads.g.doubleclick.net$|$path$|$1 & doubleclick.net      & Google LLC            & 17.025              \\
			hn                                     & doubleclick.net      & Google LLC            & 15.780              \\
			url                                    & google.com           & Google LLC            & 15.620              \\
			tiba                                   & doubleclick.net      & Google LLC            & 15.120              \\
			eid                                    & doubleclick.net      & Google LLC            & 14.585              \\
			tiba                                   & google.com           & Google LLC            & 14.310              \\
			\bottomrule
		\end{tabular}
	}
	\label{tab:top_20_decorations_negative}
\end{table}

==> graveyard/top_20_link_decorations_cookies.tex <==
\begin{table}[]
    \centering
  	\resizebox{\linewidth}{!}{\begin{tabular}{l c c c}
\toprule
         \textbf{Link} &                         \textbf{Domain} &  \textbf{Cookies} &  \textbf{Percentage} \\
        \textbf{Decoration} &                         \textbf{} &  \textbf{Sent} &  \textbf{of Sites} \\
\midrule
                cid &       www.google-analytics.com &      251 &    62.78 \\
               \_gid &       www.google-analytics.com &      206 &    55.74 \\
                cid &        stats.g.doubleclick.net &      220 &    40.65 \\
               \_gid &        stats.g.doubleclick.net &      133 &    37.11 \\
                cid &                 www.google.com &      193 &    26.31 \\
               3pid &                   ce.lijit.com &      167 &    24.54 \\
                put &       pixel.rubiconproject.com &      185 &    24.41 \\
                 id &          s.amazon-adsystem.com &      213 &    21.16 \\
  partner\_device\_id &                pixel.tapad.com &      174 &    21.04 \\
                fbp &               www.facebook.com &        5 &    19.17 \\
                  i &            usersync.gumgum.com &      138 &    18.11 \\
               xuid &                  eb2.3lift.com &      182 &    17.96 \\
                val &                 us-u.openx.net &      132 &    17.70 \\
            user\_id &                x.bidswitch.net &      139 &    17.65 \\
             userId &            ads.stickyadstv.com &      129 &    16.54 \\
             ga\_sid & securepubads.g.doubleclick.net &      618 &    16.42 \\
    piggybackCookie &           simage2.pubmatic.com &      127 &    16.10 \\
        partner\_uid &               idsync.rlcdn.com &      208 &    15.67 \\
               auid &    googleads.g.doubleclick.net &       46 &    14.55 \\
                uid &        ups.analytics.yahoo.com &      182 &    13.65 \\
\bottomrule
\end{tabular}
    

    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> graveyard/top_50_link_decorations_cookies.tex <==
\begin{table}[]
    \centering
  	\resizebox{\linewidth}{!}{\begin{tabular}{l c c c}
\toprule
         \textbf{Link} &                         \textbf{Domain} &  \textbf{Cookies} &  \textbf{\%} \\
        \textbf{Decoration} &                         \textbf{} &  \textbf{Sent} &  \textbf{of Sites} \\
\midrule
                         cid &       www.google-analytics.com &      251 &    56.83 \\
                        \_gid &       www.google-analytics.com &      206 &    50.90 \\
                         cid &        stats.g.doubleclick.net &      220 &    36.60 \\
                        \_gid &        stats.g.doubleclick.net &      133 &    34.04 \\
                         cid &                 www.google.com &      193 &    23.43 \\
                         fbp &               www.facebook.com &        5 &    19.14 \\
                        auid &    googleads.g.doubleclick.net &       46 &    13.40 \\
                         cid &           analytics.google.com &       98 &    11.03 \\
                      cookie &    googleads.g.doubleclick.net &        1 &     7.72 \\
                        gpic &    googleads.g.doubleclick.net &        1 &     7.71 \\
                      ga\_vid &    googleads.g.doubleclick.net &      112 &     6.97 \\
                      ga\_vid & securepubads.g.doubleclick.net &       54 &     6.68 \\
                      cookie &   partner.googleadservices.com &        1 &     5.60 \\
                        gpic &   partner.googleadservices.com &        1 &     5.59 \\
                         vid &                   bat.bing.com &        2 &     5.55 \\
                         sid &                   bat.bing.com &        2 &     5.54 \\
                      cookie & securepubads.g.doubleclick.net &        1 &     5.44 \\
                        gpic & securepubads.g.doubleclick.net &        1 &     5.41 \\
                         sid &       www.google-analytics.com &      802 &     4.99 \\
                     user\_id &                x.bidswitch.net &      139 &     4.69 \\
                 partner\_uid &               idsync.rlcdn.com &      208 &     4.61 \\
           partner\_device\_id &                pixel.tapad.com &      174 &     4.48 \\
                   google\_hm &           cm.g.doubleclick.net &       77 &     4.26 \\
                         uid &        ups.analytics.yahoo.com &      182 &     4.18 \\
                         put &       pixel.rubiconproject.com &      185 &     3.95 \\
                          ts &               www.facebook.com &      202 &     3.84 \\
                      ga\_sid & securepubads.g.doubleclick.net &      618 &     3.79 \\
                         rst &  pagead2.googlesyndication.com &      115 &     3.50 \\
                          it &               www.facebook.com &      167 &     3.48 \\
                        auid &                 www.google.com &       29 &     3.48 \\
                          id &          s.amazon-adsystem.com &      213 &     3.45 \\
                        info &                 gum.criteo.com &        2 &     3.30 \\
                         val &                 us-u.openx.net &      132 &     3.13 \\
pr-bh.ybp.yahoo.com||path||2 &            pr-bh.ybp.yahoo.com &       47 &     3.13 \\
                          dt & securepubads.g.doubleclick.net &      117 &     3.11 \\
                          id &               tags.bluekai.com &       90 &     3.07 \\
                         fst &    googleads.g.doubleclick.net &      188 &     3.04 \\
                      ga\_sid &    googleads.g.doubleclick.net &      741 &     2.95 \\
                    ttd\_puid &               match.adsrvr.org &       17 &     2.91 \\
                      random &    googleads.g.doubleclick.net &      182 &     2.91 \\
                        3pid &                   ce.lijit.com &      167 &     2.89 \\
                      random &                 www.google.com &      182 &     2.85 \\
            external\_user\_id &       dsum-sec.casalemedia.com &      126 &     2.84 \\
                         lmt & securepubads.g.doubleclick.net &      414 &     2.76 \\
                        xuid &                  eb2.3lift.com &      182 &     2.75 \\
                         sid &           analytics.google.com &      490 &     2.71 \\
                         dlt & securepubads.g.doubleclick.net &       66 &     2.56 \\
                          dl &       www.google-analytics.com &      214 &     2.37 \\
                         lmt &    googleads.g.doubleclick.net &      620 &     2.33 \\
                 bidder\_uuid &                    i.liadm.com &       85 &     2.28 \\
\bottomrule
\end{tabular}

}

    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> tables/decorations-most-common-feature.tex <==
\begin{table}[]
    \centering\
    \caption{Most important feature }
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l c}
    \toprule
                           Decoration Name &     Most Important Feature \\
    \midrule
           cm.g.doubleclick.net$|$google\_hm &    max\_depth\_decoration \\
                ads.google.com$|$utm\_medium &               num\_nodes \\
                ads.google.com$|$utm\_source &               num\_nodes \\
              ads.google.com$|$utm\_campaign &               num\_nodes \\
                          b.6sc.co$|$an\_uid &    max\_depth\_decoration \\
            www.google-analytics.com$|$\_gid &               num\_edges \\
             www.google-analytics.com$|$cid &    max\_depth\_decoration \\
         googleads.g.doubleclick.net$|$auid & num\_script\_predecessors \\
                adservice.google.com$|$auid &               num\_nodes \\
        securepubads.g.doubleclick.net$|$dt &               num\_edges \\
    securepubads.g.doubleclick.net$|$ga\_sid &               num\_edges \\
             stats.g.doubleclick.net$|$\_gid &    max\_depth\_decoration \\
                      www.facebook.com$|$ts &    max\_depth\_decoration \\
              stats.g.doubleclick.net$|$cid &    max\_depth\_decoration \\
       securepubads.g.doubleclick.net$|$dlt &               num\_nodes \\
                     bat.bing.com$|$msclkid &    max\_depth\_decoration \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:my_label}
\end{table}
